mRobust04: A Multilingual Version of the TREC Robust 2004 Benchmark

Robust 2004 is an information retrieval benchmark whose large number of judgments per query make it a reliable evaluation dataset. In this paper, we present mRobust04, a multilingual version of Robust04 that was translated to 8 languages using Google Translate. We also provide results of three different multilingual retrievers on this dataset. The dataset is available at https://huggingface.co/datasets/unicamp-dl/mrobust

==> table_mrobust_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{l|l|l|l|l|l} 
\toprule
Languages                   & Model    & NDCG@20 & NDCG'@20 & R@1000 & J@20    \\ 
\midrule
\multirow{3}{*}{English}    & BM25     & 0.3894  & 0.394    & 0.6495 & 0.9578  \\
                            & mT5      & 0.4661  & 0.4863   & 0.6495 & 0.8964  \\
                            & mColBERT & 0.3629  & 0.4147   & 0.5979 & 0.734   \\ 
\midrule
\multirow{3}{*}{Spanish}    & BM25     & 0.3645  & 0.3943   & 0.6405 & 0.841   \\
                            & mT5      & 0.4023  & 0.454    & 0.6405 & 0.7826  \\
                            & mColBERT & 0.3098  & 0.3898   & 0.547  & 0.635   \\ 
\midrule
\multirow{3}{*}{French}     & BM25     & 0.3896  & 0.4185   & 0.6559 & 0.8436  \\
                            & mT5      & 0.3766  & 0.4295   & 0.6559 & 0.7558  \\
                            & mColBERT & 0.3025  & 0.3835   & 0.526  & 0.6182  \\ 
\midrule
\multirow{3}{*}{Italian}    & BM25     & 0.3872  & 0.4119   & 0.6284 & 0.8482  \\
                            & mT5      & 0.3848  & 0.4364   & 0.6284 & 0.7722  \\
                            & mColBERT & 0.305   & 0.3797   & 0.5255 & 0.623   \\ 
\midrule
\multirow{3}{*}{Portuguese} & BM25     & 0.3893  & 0.4096   & 0.6572 & 0.8704  \\
                            & mT5      & 0.3917  & 0.4393   & 0.6572 & 0.777   \\
                            & mColBERT & 0.3239  & 0.4011   & 0.5491 & 0.6586  \\ 
\midrule
\multirow{3}{*}{Indonesian} & BM25     & 0.3837  & 0.407    & 0.6497 & 0.846   \\
                            & mT5      & 0.3749  & 0.4326   & 0.6497 & 0.753   \\
                            & mColBERT & 0.2876  & 0.3679   & 0.5109 & 0.6132  \\ 
\midrule
\multirow{3}{*}{German}     & BM25     & 0.3331  & 0.3727   & 0.5148 & 0.7594  \\
                            & mT5      & 0.3753  & 0.4356   & 0.5148 & 0.7294  \\
                            & mColBERT & 0.2805  & 0.3617   & 0.5039 & 0.5836  \\ 
\midrule
\multirow{3}{*}{Russian}    & BM25     & 0.3721  & 0.4039   & 0.6274 & 0.8162  \\
                            & mT5      & 0.3721  & 0.4313   & 0.6274 & 0.7314  \\
                            & mColBERT & 0.2653  & 0.3488   & 0.4751 & 0.5544  \\ 
\midrule
\multirow{3}{*}{Chinese}    & BM25     & 0.2898  & 0.3493   & 0.5173 & 0.6662  \\
                            & mT5      & 0.3586  & 0.4187   & 0.5173 & 0.7028  \\
                            & mColBERT & 0.2623  & 0.3455   & 0.4233 & 0.55    \\
\bottomrule
\end{tabular}
\caption{Results on mRobust04 multilingual dataset with mColBERT and mT5}
\label{tab:robust-multilingual}
\end{table}



==> table_mrtydi.tex <==
\begin{table}[]
\centering
\begin{tabular}{lrrrrrrrrrrr}
\hline
         & \multicolumn{1}{l}{\textit{ar}} & \multicolumn{1}{l}{\textit{bn}} & \multicolumn{1}{l}{\textit{en}} & \multicolumn{1}{l}{\textit{fi}} & \multicolumn{1}{l}{\textit{id}} & \multicolumn{1}{l}{\textit{ja}} & \multicolumn{1}{l}{\textit{ko}} & \multicolumn{1}{l}{\textit{ru}} & \multicolumn{1}{l}{\textit{sw}} & \multicolumn{1}{l}{te} & \multicolumn{1}{l}{avg} \\ \hline
\multicolumn{12}{c}{MRR@100}                                                                                                                                                                                                                                                                                                                                                  \\
BM25     & 0.562                           & 0.713                           & 0.372                           & 0.553                           & 0.661                           & 0.504                           & 0.454                           & 0.643                           & 0.662                           & 0.664                  & 0.579                   \\
mT5      & 0.736                           & 0.792                           & 0.550                           & 0.678                           & 0.753                           & 0.691                           & 0.585                           & 0.718                           & 0.762                           & 0.801                  & 0.707                   \\
mColBERT & 0.695                           & 0.742                           & 0.538                           & 0.631                           & 0.743                           & 0.575                           & 0.549                           & 0.724                           & 0.687                           & 0.778                  & 0.666                   \\ \hline
\multicolumn{12}{c}{Recall@100}                                                                                                                                                                                                                                                                                                                                               \\
BM25     & 0.933                           & 0.973                           & 0.837                           & 0.903                           & 0.952                           & 0.932                           & 0.858                           & 0.921                           & 0.878                           & 0.943                  & 0.913                   \\
mT5      & 0.957                           & 0.982                           & 0.913                           & 0.946                           & 0.976                           & 0.974                           & 0.919                           & 0.944                           & 0.910                           & 0.977                  & 0.950                   \\
mColBERT & 0.941                           & 0.973                           & 0.942                           & 0.931                           & 0.964                           & 0.836                           & 0.907                           & 0.966                           & 0.922                           & 0.991                  & 0.937                   \\ \hline
\end{tabular}
\caption{Results on document retrieval on Mr. Tydi dataset}
\label{tab:mr-tydi-parse}
\end{table}
